Lorenz equations and the figure eight knot

Lorenz equations were first presented in 1963 by Edward Lorenz, they depend on three real positive parameters. For some of these parameters which are called T-points, there are two heteroclinic orbits connecting the three singular points in the equations. The heteroclinic connections can be extended into an invariant curve passing through infinity. We consider the system at the second T-point parameter, and develop a geometric model for the flow that simulates the Lorenz dynamics there. We show that the model contains infinitely many periodic orbits, and that as knots they are all positive, prime and fibered.

==> Lorenz.tex <==
\section{Back To Lorenz System}
Assume there exist heteroclinic figure-eight parameter values for the Lorenz system, in this section we will show that the periodic orbits which appear in the Anosov flow we found has the same link of the periodic orbits which appear in the Lorenz system with heteroclinic figure-eight parameters.

\begin{theorem}
    Assume that there exists a heteroclinic figure-eight parameter for the Lorenz system. For any knot appearing as a periodic orbit on the template there exist a periodic orbit for the original equation at a figure-eight parameter with the same knot type.
\end{theorem}

\begin{proof}
    As we have mentioned before, for most of the parameter values, Lorenz system has three singular points, these singular points prevents the attractor from being hyperbolic, and they are main cause of the system instability \cite{Pinsky2017}. Therefore, in case that the heteroclinic figure-eight knot appears for such parameter values, we need to make the system stable. In order to do so, we can perform double Hopf deformation at the neighborhoods of the points $p^\pm$ as in Figure \ref{fig8.1}, the effect of such a deformation is transforming the saddle points $p^\pm$ into sinks \cite{Bonatti2021}.\\
    According to \cite{Bonatti2021}, \cite{pinsky2022around}, after performing such a deformation, we can remove a solid torus from $S^3$ by removing a three dimensional neighborhood of the figure-eight knot in the following way: start from a small neighborhood of the origin and then extend it along the separatrices, until reaching the wing centers, then connect the wing centers on the other side to the sphere around $\infty$ along the figure-eight knot.\\
    By removing the torus our flow becomes a non-singular flow on the figure-eight knot complement. Then using isotopy, we can get a hyperbolic first return map on the cross section $R$.\\
    \begin{figure}[h]
        \centering
        \includegraphics[width=8cm]{Figures/Fig8.1.png}
        \caption{Hopf bifurcation}
        \label{fig8.1}
    \end{figure}
    By applying an isotopy on the cross section $R$ which makes the first return map hyperbolic, we get the existence of two directions in the two-dimensional cross section which are preserved under the flow, one direction uniformly expands and the other direction uniformly contracts under the hyperbolic first return map.
    This yields a geometric model \ref{fig5} for the figure-eight T-point which can be achieved by taking the hyperbolic first return map, and using all the properties that we have proved over the heteroclinic orbits in section $4$. 
    \begin{figure}[!h]
        \centering
        \includegraphics[width=8cm]{Figures/Fig5.1.jpg}
        \caption{The geometric model}
        \label{fig5}
    \end{figure}
    Since the first return map became hyperbolic, we can find a template that carries all the periodic orbits of the flow. Such a template can be obtained by collapsing the geometric model over the contracting direction i.e. the stable direction, doing that we get the same template we saw in section $5$ (see Figure \ref{fig6}).\\
    The last thing that we need to prove is that the periodic orbits which appear on the template, i.e. the periodic orbits of the hyperbolic flow, appears also in the system at a figure-eight T-point. In order to prove that, we will use Theorem \ref{thmpa}, we embed the hyperbolic first return map into a diffeomorphism of a closed 2-dimensional surface, our surface will be a four punctured Mobius strip. We choose a graph that is a spine for the surface consisting of eight edges, each edge represents a different part of the cross section $R$ after collapsing over the stable direction: blue - part $A$, green - part $B$, orange - part $C$, red - part $D$, yellow - the stable manifold of the origin (see Figure \ref{fig8.3}), black and grey edges which we add in order to have only vertices of order three.
    \begin{figure}[!h]
        \centering
        \includegraphics[width=10cm]{Figures/Fig8.4.jpg}
        \caption{(a) The cross section $R$ is divided into four parts $A,B,C$ and $D$. (b) The images of parts $A,B,C$ and $D$ under the hyperbolic first return map.}
        \label{fig8.3}
    \end{figure}
    
    The action of the map on the graph is given in Figure \ref{fig8.2}. This action defines a diffeomorphism on the four punctured Mobius strip,
    we can choose a hyperbolic first return map on $R$ such that the unstable direction contracts by $\lambda$ and the stable direction expands by $\lambda$, these directions are transverse which implies that $\phi$ is pseudo Anosov on a closed 2-dimensional manifold, therefore, by Theorem \ref{thmpa}, any periodic orbit of $\phi$ is isotopic stable.\\
    Periodic orbits on the template are in one to one correspondence with periodic orbits of $\phi$ passing only in $A, B, C, D$. So they are isotopy stable and exist also for the original return map.

    \begin{figure}
        \centering
        \includegraphics[width=10cm]{Figures/Fig8.2.jpg}
        \caption{The action of the map on the graph}
        \label{fig8.2}
    \end{figure}
\end{proof}
